Optimal Rates for Federated Variational Inequalities under different relaxations of bounded variance assumption

We study how interpolation affects local steps and parallel sampling in monotone variational inequalities (VIs), with $m$ workers, $K$ oracle calls per worker per round, and $N$ rounds. Under the strong growth condition (SGC), we determine the minimax rate for affine VIs, attained by local extragradient with worker averaging. For nonlinear monotone VIs and convex-concave saddle problems with Lipschitz operators satisfying SGC, we improve the stochastic terms of bounded-variance expected-gap guarantees from $(KN)^{-1/2}$ to $(KN)^{-1}$ with local steps and from $(mKN)^{-1/2}$ to $(mKN)^{-1}$ with minibatches. Under strong monotonicity, we improve the noise-dependent condition-number scaling of existing extragradient bounds from quadratic to linear. The resulting monotone-gap and strongly monotone accuracy bounds match lower bounds up to logarithmic factors in $m$. Under generalized smoothness and SGC, adaptive steps give polynomial dependence on the initial radius. For affine VIs with globally bounded oracle variance, we also attain the minimax rate: the deterministic rate over $KN$ sequential calls plus the statistical rate over all $mKN$ samples. For composite VIs with smooth convex sample interpolation and an exactly evaluated monotone Lipschitz component, accelerated mirror-prox sliding achieves an $N^{-2}$ gradient term, a $(KN)^{-1}$ monotone term, and a $(mKN)^{-1}$ sampling term, without assuming SGC.

==> appendices/contents.tex <==
\makeatletter
\section*{Appendix contents}
\begingroup
\small
\setcounter{tocdepth}{3}
\renewcommand*\l@section[2]{%
  \ifnum\c@tocdepth>\z@
    \addpenalty\@secpenalty
    \addvspace{.7em\@plus\p@}%
    \setlength\@tempdima{2em}%
    \begingroup
      \parindent\z@ \rightskip\@pnumwidth
      \parfillskip-\@pnumwidth
      \leavevmode\bfseries
      \advance\leftskip\@tempdima \hskip-\leftskip
      #1\nobreak\hfil\nobreak
      \hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
    \penalty\@M
  \fi}
\renewcommand*\l@subsection{\@dottedtocline{2}{2em}{3em}}
\renewcommand*\l@subsubsection{\@dottedtocline{3}{5em}{3.5em}}
\hypersetup{linktoc=all}
\@starttoc{aptoc}
\endgroup
% Record appendix headings separately while preserving the PDF bookmarks.
\let\appendix@addcontentsline\addcontentsline
\renewcommand{\addcontentsline}[3]{%
  \appendix@addcontentsline{#1}{#2}{#3}%
  \def\appendix@entrytype{#1}%
  \def\appendix@tocname{toc}%
  \ifx\appendix@entrytype\appendix@tocname
    \addtocontents{aptoc}{%
      \protect\contentsline{#2}{#3}{\thepage}{\@currentHref}\protected@file@percent}%
  \fi
}
\makeatother
\clearpage

